Physics informed machine learning with Smoothed Particle Hydrodynamics: Hierarchy of reduced Lagrangian models of turbulence

Building efficient, accurate and generalizable reduced order models of developed turbulence remains a major challenge. This manuscript approaches this problem by developing a hierarchy of parameterized reduced Lagrangian models for turbulent flows, and investigates the effects of enforcing physical structure through Smoothed Particle Hydrodynamics (SPH) versus relying on neural networks (NN)s as universal function approximators. Starting from Neural Network (NN) parameterizations of a Lagrangian acceleration operator, this hierarchy of models gradually incorporates a weakly compressible and parameterized SPH framework, which enforces physical symmetries, such as Galilean, rotational and translational invariances. Within this hierarchy, two new parameterized smoothing kernels are developed in order to increase the flexibility of the learn-able SPH simulators. For each model we experiment with different loss functions which are minimized using gradient based optimization, where efficient computations of gradients are obtained by using Automatic Differentiation (AD) and Sensitivity Analysis (SA). Each model within the hierarchy is trained on two data sets associated with weekly compressible Homogeneous Isotropic Turbulence (HIT): (1) a validation set using weakly compressible SPH; and (2) a high fidelity set from Direct Numerical Simulations (DNS). Numerical evidence shows that encoding more SPH structure improves generalizability to different turbulent Mach numbers and time shifts, and that including the novel parameterized smoothing kernels improves the accuracy of SPH at the resolved scales.

==> sections_response/related_work.tex <==


\section{Physics Informed Machine Learning: Related Work}
\label{sec:related_work}


Early work incorporating scientific domain knowledge (e.g. from physics in the form of differential equations) and computational scheme (collocation method for solving the differential equations)  within machine learning algorithms dates back to the 1990s \cite{Lagaris_nn_ode98}. However, in the context of modern machine learning and specifically deep learning, interest in this area has been revived \cite{raissi2, node, rackauckas2020universal, ladicky2015_Rforests}. In part, this is due to the increased computational power afforded by parallelism across both CPUs and GPUs, along with notable achievements across disciplines (such as scientific applications \cite{sci_ml_applications}, data-compression algorithms \cite{WANG2016}, computer vision \cite{serre_deep_learning_mv}, and natural language processing \cite{nlp_book}. The main computational utilities and strategies of the Physics Informed Machine Learning (PIML) includes embedding physical structure into learn-able models, applying NNs as function approximators \cite{hornik_nn_approx89}, differential programming using automatic differentiation \cite{rackauckas2020universal, ad_bucker06}, and optimization tools to minimize an objective (loss) function. 

There are several approaches that can be taken to develop a PIML algorithm; (1) enforcing soft constraints by adding physical structure, or symmetries into the loss function (as was done in \cite{raissi2} where Neural Networks are used to discover and solve parameterized PDEs from data); (2) enforce physical constraints directly into the NN architecture (such as in \cite{mohanNN} enforced the incompressiblility constraint into a Convolutional NN); (3) utilize NN's as function approximators along with physical parameters/structure embedded within  differentiable numerical simulators (as was done in \cite{node, rackauckas2020universal,2021Yifeng-PRF}); (4) mixing differentiable programming with SA along with physical structure and NNs as was done by \cite{ma2021comparison, node} (which from a technical perspective is most related to our work). The methods of this work is most related to (4) as an approach to build parameterized reduced Lagrangian models for turbulence. In this manuscript, we combine these scientific disciplines to not only provide a tool for approaching the discovery of optimal Lagrangian and SPH based models of turbulence, but also to explore the effects of adding physical structure into machine learning algorithms to extrapolate and generalize beyond the regimes available for training.

In this manuscript we focus specifically on building PIML scheme(s) which are taking advantage of the Lagrangian representation of the flows. 
%In recent years, there have been several works that have integrated machine learning and deep learning techniques for Lagrangian flows. 
One of the earliest contributions to this field was made in \cite{ladicky2015_Rforests} where SPH related models were used along side with the regression forest technique of the machine learning. It was demonstrated in this work that physics informed feature vectors helps to represent turbulent flows efficiently. In another relevant work \cite{suare2018_evolution} evolutionary algorithms were applied to optimize parameters in SPH flows. Differentiable programming techniques were utilized in \cite{schenck2018_spnet} for Lagrangian robotic control of flows and in \cite{Ummenhofer2020conv} where a continuous convolutional Neural Network (NN) approach was developed to train SPH on the multi-particle Lagrangian data. NNs were utilized in \cite{2021Yifeng-PRF} to train a closure model for Lagrangian dynamics of the velocity gradient tensor in homogeneous isotropic turbulence on the Direct Numerical Simulation (DNS) data. NNs were also used in \cite{rabault2017performing,lee2017piv,cai2019particle,stulov2021neural} to improve Particle Image Velocimetry techniques using experimental data to map Lagrangian representation of the flow (trajectories of particles)  into its Eulerian counterpart (velocity field).  Most recent, and related to this work, in \cite{tian_22_LLES} Tian et al. developed a fully differentiable and generalized Lagrangian Large Eddy Simulator capable of fitting and generalizing to high fidelity DNS data.

%\cite{2021Yifeng-PRF} learns reduced models describing Lagrangian dynamics of the velocity gradient tensor from Direct Numerical Simulation (DNS) data. 
%operation were developed on unordered particle data for learning and simulating SPH.
%Further works began utilizing differentiable programming techniques, such as in \cite{schenck2018_spnet} for robotic control for pouring applications and in \cite{Ummenhofer2020conv} where a continuous convolutional neural network operation were developed on unordered particle data for learning and simulating SPH.

